Verifying Temporal Properties of Reactive Systems by Transformation

We show how program transformation techniques can be used for the verification of both safety and liveness properties of reactive systems. In particular, we show how the program transformation technique distillation can be used to transform reactive systems specified in a functional language into a simplified form that can subsequently be analysed to verify temporal properties of the systems. Example systems which are intended to model mutual exclusion are analysed using these techniques with respect to both safety (mutual exclusion) and liveness (non-starvation), with the errors they contain being correctly identified.

==> eptcsdata.tex <==
\providecommand{\firstpage}{33}
\providecommand{\publicationstatus}{A. Lisitsa, A.P. Nemytykh, A. Pettorossi (Eds.): 3rd International Workshop\\ on Verification and Program Transformation (VPT 2015)\\
EPTCS 199, 2015, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.199.3}{10.4204/EPTCS.199.3}}

